Causal Inference with Invalid Instruments: Post-selection Problems and A Solution Using Searching and Sampling

Instrumental variable methods are among the most commonly used causal inference approaches to deal with unmeasured confounders in observational studies. The presence of invalid instruments is the primary concern for practical applications, and a fast-growing area of research is inference for the causal effect with possibly invalid instruments. This paper illustrates that the existing confidence intervals may undercover when the valid and invalid instruments are hard to separate in a data-dependent way. To address this, we construct uniformly valid confidence intervals that are robust to the mistakes in separating valid and invalid instruments. We propose to search for a range of treatment effect values that lead to sufficiently many valid instruments. We further devise a novel sampling method, which, together with searching, leads to a more precise confidence interval. Our proposed searching and sampling confidence intervals are uniformly valid and achieve the parametric length under the finite-sample majority and plurality rules. We apply our proposal to examine the effect of education on earnings. The proposed method is implemented in the R package RobustIV available from CRAN.

==> IVRef_full.tex <==
@article{guo2022two,
  title={Two Stage Curvature Identification with Machine Learning: Causal Inference with Possibly Invalid Instrumental Variables},
  author={Guo, Zijian and B{\"u}hlmann, Peter},
  journal={arXiv preprint arXiv:2203.12808},
  year={2022}
}
@article{xie2022repro,
  title={Repro Samples Method for Finite-and Large-Sample Inferences},
  author={Xie, Min-ge and Wang, Peng},
  journal={arXiv preprint arXiv:2206.06421},
  year={2022}
}
@article{goh2022causal,
  title={Causal inference with some invalid instrumental variables: A quasi-Bayesian approach},
  author={Goh, Gyuhyeong and Yu, Jisang},
  journal={Oxford Bulletin of Economics and Statistics},
  volume={84},
  number={6},
  pages={1432--1451},
  year={2022},
  publisher={Wiley Online Library}
}
@article{liao2013adaptive,
  title={Adaptive GMM shrinkage estimation with consistent moment selection},
  author={Liao, Zhipeng},
  journal={Econometric Theory},
  volume={29},
  number={5},
  pages={857--904},
  year={2013},
  publisher={Cambridge University Press}
}
@article{cheng2015select,
  title={Select the valid and relevant moments: An information-based LASSO for GMM with many moments},
  author={Cheng, Xu and Liao, Zhipeng},
  journal={Journal of Econometrics},
  volume={186},
  number={2},
  pages={443--464},
  year={2015},
  publisher={Elsevier}
}
@article{hahn2005estimation,
  title={Estimation with valid and invalid instruments},
  author={Hahn, Jinyong and Hausman, Jerry},
  journal={Annales d'Economie et de Statistique},
  pages={25--57},
  year={2005},
  publisher={JSTOR}
}
@article{guggenberger2012asymptotic,
  title={On the asymptotic size distortion of tests when instruments locally violate the exogeneity assumption},
  author={Guggenberger, Patrik},
  journal={Econometric Theory},
  volume={28},
  number={2},
  pages={387--421},
  year={2012},
  publisher={Cambridge University Press}
}
@article{berkowitz2012validity,
  title={The validity of instruments revisited},
  author={Berkowitz, Daniel and Caner, Mehmet and Fang, Ying},
  journal={Journal of Econometrics},
  volume={166},
  number={2},
  pages={255--266},
  year={2012},
  publisher={Elsevier}
}
@article{caner2018adaptive,
  title={Adaptive elastic net gmm estimation with many invalid moment conditions: Simultaneous model and moment selection},
  author={Caner, Mehmet and Han, Xu and Lee, Yoonseok},
  journal={Journal of Business \& Economic Statistics},
  volume={36},
  number={1},
  pages={24--46},
  year={2018},
  publisher={Taylor \& Francis}
}
@article{belloni2014inference,
  title={Inference on treatment effects after selection among high-dimensional controls},
  author={Belloni, Alexandre and Chernozhukov, Victor and Hansen, Christian},
  journal={The Review of Economic Studies},
  volume={81},
  number={2},
  pages={608--650},
  year={2014},
  publisher={Oxford University Press}
}
@article{xie2012china,
  title={China family panel studies (2010) user’s manual},
  author={Xie, Yu},
  journal={Beijing: Institute of Social Science Survey, Peking University},
  year={2012}
}
@article{behrman2012financial,
  title={How financial literacy affects household wealth accumulation},
  author={Behrman, Jere R and Mitchell, Olivia S and Soo, Cindy K and Bravo, David},
  journal={American Economic Review},
  volume={102},
  number={3},
  pages={300--304},
  year={2012}
}
@article{blackburn1993omitted,
  title={Omitted-ability bias and the increase in the return to schooling},
  author={Blackburn, McKinley L and Neumark, David},
  journal={Journal of labor economics},
  volume={11},
  number={3},
  pages={521--544},
  year={1993},
  publisher={University of Chicago Press}
}
@article{trostel2002estimates,
  title={Estimates of the economic return to schooling for 28 countries},
  author={Trostel, Philip and Walker, Ian and Woolley, Paul},
  journal={Labour economics},
  volume={9},
  number={1},
  pages={1--16},
  year={2002},
  publisher={Elsevier}
}
@article{bhatti2013economic,
  title={Economic returns to education in France: OLS and instrumental variable estimations},
  author={Bhatti, Sajjad Haider and Bourdon, Jean and Aslam, Muhammad},
  journal={The Lahore Journal of Economics},
  volume={18},
  number={2},
  pages={51},
  year={2013},
  publisher={Lahore School of Economics}
}
@article{stock2002survey,
  title={A survey of weak instruments and weak identification in generalized method of moments},
  author={Stock, James H and Wright, Jonathan H and Yogo, Motohiro},
  journal={Journal of Business \& Economic Statistics},
  volume={20},
  number={4},
  pages={518--529},
  year={2002},
  publisher={Taylor \& Francis}
}
@article{staiger1997instrumental,
  title={Instrumental Variables Regression with Weak Instruments},
  author={Staiger, Douglas and Stock, James H},
  journal={Econometrica: Journal of the Econometric Society},
  pages={557--586},
  year={1997},
  publisher={JSTOR}
}
@article{armstrong2020bias,
  title={Bias-aware inference in regularized regression models},
  author={Armstrong, Timothy B and Koles{\'a}r, Michal and Kwon, Soonwoo},
  journal={arXiv preprint arXiv:2012.14823},
  year={2020}
}
@article{bekker2015jackknife,
  title={Jackknife instrumental variable estimation with heteroskedasticity},
  author={Bekker, Paul A and Crudu, Federico},
  journal={Journal of econometrics},
  volume={185},
  number={2},
  pages={332--342},
  year={2015},
  publisher={Elsevier}
}
@inproceedings{eicker1967limit,
  title={Limit theorems for regression with uneqaul and dependent errors},
  author={Eicker, F},
  booktitle={Proc. Fifth Berkeley Symp. Statist. Prodab.},
  pages={59--82},
  year={1967}
}
@inproceedings{huber1967under,
  title={Under nonstandard conditions},
  author={Huber, Peter J},
  booktitle={Proceedings of the Fifth Berkeley Symposium on Mathematical Statistics and Probability: Weather Modification; University of California Press: Berkeley, CA, USA},
  pages={221},
  year={1967}
}
@article{white1980heteroskedasticity,
  title={A heteroskedasticity-consistent covariance matrix estimator and a direct test for heteroskedasticity},
  author={White, Halbert},
  journal={Econometrica: journal of the Econometric Society},
  pages={817--838},
  year={1980},
  publisher={JSTOR}
}
@article{leeb2005model,
  title={Model selection and inference: Facts and fiction},
  author={Leeb, Hannes and P{\"o}tscher, Benedikt M},
  journal={Econometric Theory},
  pages={21--59},
  year={2005},
  publisher={JSTOR}
}
@article{donoho1994minimax,
  title={Minimax risk overl p-balls forl p-error},
  author={Donoho, David L and Johnstone, Iain M},
  journal={Probability Theory and Related Fields},
  volume={99},
  number={2},
  pages={277--303},
  year={1994},
  publisher={Springer}
}
@article{donoho1994ideal,
  title={Ideal spatial adaptation by wavelet shrinkage},
  author={Donoho, David L and Johnstone, Jain M},
  journal={biometrika},
  volume={81},
  number={3},
  pages={425--455},
  year={1994},
  publisher={Oxford University Press}
}
@article{zhao2020statistical,
  title={Statistical inference in two-sample summary-data Mendelian randomization using robust adjusted profile score},
  author={Zhao, Qingyuan and Wang, Jingshu and Hemani, Gibran and Bowden, Jack and Small, Dylan S},
  journal={The Annals of Statistics},
  volume={48},
  number={3},
  pages={1742--1769},
  year={2020},
  publisher={Institute of Mathematical Statistics}
}
@article{hartwig2017robust,
  title={Robust inference in summary data Mendelian randomization via the zero modal pleiotropy assumption},
  author={Hartwig, Fernando Pires and Davey Smith, George and Bowden, Jack},
  journal={International journal of epidemiology},
  volume={46},
  number={6},
  pages={1985--1998},
  year={2017},
  publisher={Oxford University Press}
}
@article{wang2020repro,
  title={Repro Sampling Method for Statistical Inference of High Dimensional Linear Models},
  author={Wang, Peng and Xie, Minge},
  journal={Research Manuscript},
  year={2020}
}
@article{liu2020mendelian,
  title={On Mendelian Randomization Mixed-Scale Treatment Effect Robust Identification (MR MiSTERI) and Estimation for Causal Inference},
  author={Liu, Zhonghua and Ye, Ting and Sun, Baoluo and Schooling, Mary and Tchetgen, Eric Tchetgen},
  journal={arXiv preprint arXiv:2009.14484},
  year={2020}
}

@article{han2008detecting,
  title={Detecting invalid instruments using L1-GMM},
  author={Han, Chirok},
  journal={Economics Letters},
  volume={101},
  number={3},
  pages={285--287},
  year={2008},
  publisher={Elsevier}
}
@article{small2007sensitivity,
  title={Sensitivity analysis for instrumental variables regression with overidentifying restrictions},
  author={Small, Dylan S},
  journal={Journal of the American Statistical Association},
  volume={102},
  number={479},
  pages={1049--1058},
  year={2007},
  publisher={Taylor \& Francis}
}
@article{lee2016exact,
  title={Exact post-selection inference, with application to the lasso},
  author={Lee, Jason D and Sun, Dennis L and Sun, Yuekai and Taylor, Jonathan E},
  journal={Annals of Statistics},
  volume={44},
  number={3},
  pages={907--927},
  year={2016},
  publisher={Institute of Mathematical Statistics}
}
@article{lewbel2018identification,
  title={Identification and estimation using heteroscedasticity without instruments: The binary endogenous regressor case},
  author={Lewbel, Arthur},
  journal={Economics Letters},
  volume={165},
  pages={10--12},
  year={2018},
  publisher={Elsevier}
}
@article{tchetgen2017genius,
  title={The GENIUS approach to robust Mendelian randomization inference},
  author={Tchetgen, Eric J Tchetgen and Sun, BaoLuo and Walter, Stefan},
  journal={arXiv preprint arXiv:1709.07779},
  year={2017}
}
@article{spiller2019detecting,
  title={Detecting and correcting for bias in Mendelian randomization analyses using Gene-by-Environment interactions},
  author={Spiller, Wes and Slichter, David and Bowden, Jack and Davey Smith, George},
  journal={International journal of epidemiology},
  volume={48},
  number={3},
  pages={702--712},
  year={2019},
  publisher={Oxford University Press}
}

@article{windmeijer2019use,
  title={On the use of the lasso for instrumental variables estimation with some invalid instruments},
  author={Windmeijer, Frank and Farbmacher, Helmut and Davies, Neil and Davey Smith, George},
  journal={Journal of the American Statistical Association},
  volume={114},
  number={527},
  pages={1339--1350},
  year={2019},
  publisher={Taylor \& Francis}
}
@article{bowden2015mendelian,
  title={Mendelian randomization with invalid instruments: effect estimation and bias detection through Egger regression},
  author={Bowden, Jack and Davey Smith, George and Burgess, Stephen},
  journal={International journal of epidemiology},
  volume={44},
  number={2},
  pages={512--525},
  year={2015},
  publisher={Oxford University Press}
}

@article{hansen1982large,
  title={Large sample properties of generalized method of moments estimators},
  author={Hansen, Lars Peter},
  journal={Econometrica: Journal of the Econometric Society},
  pages={1029--1054},
  year={1982},
  publisher={JSTOR}
}
@article{sargan1958estimation,
  title={The estimation of economic relationships using instrumental variables},
  author={Sargan, John D},
  journal={Econometrica: Journal of the Econometric Society},
  pages={393--415},
  year={1958},
  publisher={JSTOR}
}
@article{Kang16,
  title={Instrumental variables estimation with some invalid instruments and its application to Mendelian randomization},
  author={Kang, Hyunseung and Zhang, Anru and Cai, T Tony and Small, Dylan S},
  journal={Journal of the American Statistical Association},
  volume={111},
  number={513},
  pages={132--144},
  year={2016},
  publisher={Taylor \& Francis}
}
@article{fan2020endogenous,
  title={Endogenous Treatment Effect Estimation with some Invalid and Irrelevant Instruments},
  author={Fan, Qingliang and Wu, Yaqian},
  journal={arXiv preprint arXiv:2006.14998},
  year={2020}
}
@article{MR-Presso,
  title={Detection of widespread horizontal pleiotropy in causal relationships inferred from Mendelian randomization between complex traits and diseases},
  author={Verbanck, Marie and Chen, Chia-yen and Neale, Benjamin and Do, Ron},
  journal={Nature genetics},
  volume={50},
  number={5},
  pages={693--698},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{Bowden15,
  title={Mendelian randomization with invalid instruments: effect estimation and bias detection through Egger regression},
  author={Bowden, Jack and Davey Smith, George and Burgess, Stephen},
  journal={International journal of epidemiology},
  volume={44},
  number={2},
  pages={512--525},
  year={2015},
  publisher={Oxford University Press}
}

@article{Kole15,
  title={Identification and inference with many invalid instruments},
  author={Koles{\'a}r, Michal and Chetty, Raj and Friedman, John and Glaeser, Edward and Imbens, Guido W},
    journal={Journal of Business \& Economic Statistics},
  volume={33},
  number={4},
  pages={474--484},
  year={2015},
  publisher={Taylor \& Francis}
}

@article{Bowden16,
  title={Consistent estimation in Mendelian randomization with some invalid instruments using a weighted median estimator},
 author={Bowden, Jack and Davey Smith, George and Haycock, Philip C and Burgess, Stephen},
  journal={Genetic epidemiology},
  volume={40},
  number={4},
  pages={304--314},
  year={2016},
  publisher={Wiley Online Library}
}

@article{Bowden17,
  title={Robust inference in summary data Mendelian randomization via the zero modal pleiotropy assumption},
  author={Hartwig, Fernando Pires and Davey Smith, George and Bowden, Jack},
  journal={International journal of epidemiology},
  volume={46},
  number={6},
  pages={1985--1998},
  year={2017},
  publisher={Oxford University Press}
}

@article{Dylan17,
  title={A review of instrumental variable estimators for Mendelian randomization},
  author={Burgess, Stephen and Small, Dylan S and Thompson, Simon G},
  journal={Statistical methods in medical research},
  volume={26},
  number={5},
  pages={2333--2355},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{Davey03,
  title={Mendelian randomization: can genetic epidemiology contribute to understanding environmental determinants of disease?},
  author={Davey Smith, George and Ebrahim, Shah},
  journal={International journal of epidemiology},
  volume={32},
  number={1},
  pages={1--22},
  year={2003},
  publisher={Oxford University Press}
}
@article{Davey14,
  title={Mendelian randomization: genetic anchors for causal inference in epidemiological studies},
  author={Davey Smith, George and Hemani, Gibran},
  journal={Human molecular genetics},
  volume={23},
  number={R1},
  pages={R89--R98},
  year={2014},
  publisher={Oxford University Press}
}

@book{imbens2015causal,
  title={Causal inference in statistics, social, and biomedical sciences},
  author={Imbens, Guido W and Rubin, Donald B},
  year={2015},
  publisher={Cambridge University Press}
}
@book{wooldridge2010econometric,
  title={Econometric analysis of cross section and panel data},
  author={Wooldridge, Jeffrey M},
  year={2010},
  publisher={MIT press}
}

@article{kang2020two,
  title={Two robust tools for inference about causal effects with invalid instruments},
  author={Kang, Hyunseung and Lee, Youjin and Cai, T Tony and Small, Dylan S},
  journal={Biometrics},
  year={2020},
  publisher={Wiley Online Library}
}
@article{berk2013valid,
  title={Valid post-selection inference},
  author={Berk, Richard and Brown, Lawrence and Buja, Andreas and Zhang, Kai and Zhao, Linda},
  journal={The Annals of Statistics},
  volume={41},
  number={2},
  pages={802--837},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@article{li2020causal,
  title={Causal Inference for Nonlinear Outcome Models with Possibly Invalid Instrumental Variables},
  author={Li, Sai and Guo, Zijian},
  journal={arXiv preprint arXiv:2010.09922},
  year={2020}
}
@article{guo2020inference,
  title={Inference for High-dimensional Maximin Effects in Heterogeneous Regression Models Using a Sampling Approach},
  author={Guo, Zijian},
  journal={arXiv preprint arXiv:2011.07568},
  year={2020}
}
@article{anderson1949estimation,
  title={Estimation of the parameters of a single equation in a complete system of stochastic equations},
  author={Anderson, Theodore W and Rubin, Herman},
  journal={Annals of Mathematical statistics},
  volume={20},
  number={1},
  pages={46--63},
  year={1949},
  publisher={Institute of Mathematical Statistics}
}
@article{windmeijer2019confidence,
  title={The confidence interval method for selecting valid instrumental variables},
  author={Windmeijer, Frank and Liang, Xiaoran and Hartwig, Fernando P and Bowden, Jack},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={83},
  number={4},
  pages={752--776},
  year={2021},
  publisher={Wiley Online Library}
}
@article{mikusheva2013survey,
  title={Survey on statistical inferences in weakly-identified instrumental variable models},
  author={Mikusheva, Anna},
  journal={Applied Econometrics},
  volume={29},
  number={1},
  pages={117--131},
  year={2013},
  publisher={Publishing House" SINERGIA PRESS"}
}
@article{chernozhukov2015valid,
  title={Valid post-selection and post-regularization inference: An elementary, general approach},
  author={Chernozhukov, Victor and Hansen, Christian and Spindler, Martin},
  journal={Annu. Rev. Econ.},
  volume={7},
  number={1},
  pages={649--688},
  year={2015},
  publisher={Annual Reviews}
}
@article{lindsay1994efficiency,
  title={Efficiency versus robustness: the case for minimum Hellinger distance and related methods},
  author={Lindsay, Bruce G},
  journal={The Annals of Statistics},
  volume={22},
  number={2},
  pages={1081--1114},
  year={1994},
  publisher={Institute of Mathematical Statistics}
}
@article{liu1992efficiency,
  title={Efficiency and robustness in resampling},
  author={Liu, Regina Y and Singh, Kesar},
  journal={The Annals of Statistics},
  volume={20},
  number={1},
  pages={370--384},
  year={1992},
  publisher={Institute of Mathematical Statistics}
}
@article{meinshausen2006quantile,
  title={Quantile regression forests},
  author={Meinshausen, Nicolai},
  journal={Journal of Machine Learning Research},
  volume={7},
  number={Jun},
  pages={983--999},
  year={2006}
}
@article{lin2006random,
  title={Random forests and adaptive nearest neighbors},
  author={Lin, Yi and Jeon, Yongho},
  journal={Journal of the American Statistical Association},
  volume={101},
  number={474},
  pages={578--590},
  year={2006},
  publisher={Taylor \& Francis}
}
@article{kolesar2015identification,
  title={Identification and inference with many invalid instruments},
  author={Koles{\'a}r, Michal and Chetty, Raj and Friedman, John and Glaeser, Edward and Imbens, Guido W},
  journal={Journal of Business \& Economic Statistics},
  volume={33},
  number={4},
  pages={474--484},
  year={2015},
  publisher={Taylor \& Francis}
}
@techreport{windmeijer2018confidence,
  title={The Confidence Interval Method for Selecting Valid Instruments},
  author={Windmeijer, F and Liang, X and Hartwig, F and Bowden, J},
  year={2018},
  institution={Technical report, University of Bristol}
}
@article{rudelson2013hanson,
  title={Hanson-Wright inequality and sub-gaussian concentration},
  author={Rudelson, Mark and Vershynin, Roman},
  journal={Electronic Communications in Probability},
  volume={18},
  year={2013},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@inproceedings{gretton2008kernel,
  title={A kernel statistical test of independence},
  author={Gretton, Arthur and Fukumizu, Kenji and Teo, Choon H and Song, Le and Sch{\"o}lkopf, Bernhard and Smola, Alex J},
  booktitle={Advances in neural information processing systems},
  pages={585--592},
  year={2008}
}
@inproceedings{gretton2005measuring,
  title={Measuring statistical dependence with Hilbert-Schmidt norms},
  author={Gretton, Arthur and Bousquet, Olivier and Smola, Alex and Sch{\"o}lkopf, Bernhard},
  booktitle={International conference on algorithmic learning theory},
  pages={63--77},
  year={2005},
  organization={Springer}
}
@article{gretton2010consistent,
  title={Consistent nonparametric tests of independence},
  author={Gretton, Arthur and Gy{\"o}rfi, L{\'a}szl{\'o}},
  journal={Journal of Machine Learning Research},
  volume={11},
  number={Apr},
  pages={1391--1423},
  year={2010}
}
@inproceedings{gretton2008nonparametric,
  title={Nonparametric independence tests: Space partitioning and kernel approaches},
  author={Gretton, Arthur and Gy{\"o}rfi, L{\'a}szl{\'o}},
  booktitle={International Conference on Algorithmic Learning Theory},
  pages={183--198},
  year={2008},
  organization={Springer}
}
@article{gretton2005kernel,
  title={Kernel methods for measuring independence},
  author={Gretton, Arthur and Herbrich, Ralf and Smola, Alexander and Bousquet, Olivier and Sch{\"o}lkopf, Bernhard},
  journal={Journal of Machine Learning Research},
  volume={6},
  number={Dec},
  pages={2075--2129},
  year={2005}
}
@article{lewbel2012using,
  title={Using heteroscedasticity to identify and estimate mismeasured and endogenous regressor models},
  author={Lewbel, Arthur},
  journal={Journal of Business \& Economic Statistics},
  volume={30},
  number={1},
  pages={67--80},
  year={2012},
  publisher={Taylor \& Francis}
}
@article{shang2013local,
  title={Local and global asymptotic inference in smoothing spline models},
  author={Shang, Zuofeng and Cheng, Guang},
  journal={The Annals of Statistics},
  volume={41},
  number={5},
  pages={2608--2638},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}

@article{muller2015partial,
  title={The partial linear model in high dimensions},
  author={M{\"u}ller, Patric and Geer, Sara},
  journal={Scandinavian Journal of Statistics},
  volume={42},
  number={2},
  pages={580--608},
  year={2015},
  publisher={Wiley Online Library}
}

@article{shang2013localsup,
  title={Supplement to ``Local and global asymptotic inference in smoothing spline models"},
  author={Shang, Zuofeng and Cheng, Guang},
  journal={The Annals of Statistics},
  volume={41},
  number={5},
  pages={2608--2638},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}

@article {baraud2004,
AUTHOR = {Baraud, Y.},
TITLE = {Confidence balls in {G}aussian regression},
JOURNAL = {Ann. Statist.},
FJOURNAL = {The Annals of Statistics},
VOLUME = {32},
YEAR = {2004},
NUMBER = {2},
PAGES = {528--551}
}

@article {Bickel1988,
AUTHOR = {Bickel, P. J. and Ritov, Y.},
TITLE = {Estimating integrated squared density derivatives: sharp best
              order of convergence estimates},
JOURNAL = {Sankhy\=a Ser. A},
FJOURNAL = {Sankhy\=a (Statistics). The Indian Journal of Statistics.
              Series A},
VOLUME = {50},
YEAR = {1988},
NUMBER = {3},
PAGES = {381--393}
}

@article {CaiLow2006CBall,
AUTHOR = {Cai, T. Tony and Low, Mark G.},
TITLE = {Adaptive confidence balls},
JOURNAL = {Ann. Statist.},
FJOURNAL = {The Annals of Statistics},
VOLUME = {34},
YEAR = {2006},
NUMBER = {1},
PAGES = {202--228}
}

@article {dumbgen1998,
AUTHOR = {D{\"u}mbgen, L.},
TITLE = {New goodness-of-fit tests and their application to
              nonparametric confidence sets},
JOURNAL = {Ann. Statist.},
FJOURNAL = {The Annals of Statistics},
VOLUME = {26},
YEAR = {1998},
NUMBER = {1},
PAGES = {288--314}
}

@article {Genovese2005,
AUTHOR = {Genovese, C. R. and Wasserman, L.},
TITLE = {Confidence sets for nonparametric wavelet regression},
JOURNAL = {Ann. Statist.},
FJOURNAL = {The Annals of Statistics},
VOLUME = {33},
YEAR = {2005},
NUMBER = {2},
PAGES = {698--729}
}

@book {ingster2003,
AUTHOR = {Ingster, Y. I. and Suslina, I. A.},
TITLE = {Nonparametric goodness-of-fit testing under {G}aussian models},
SERIES = {Lecture Notes in Statistics},
VOLUME = {169},
PUBLISHER = {Springer-Verlag, New York},
YEAR = {2003}
}

@article {lepski1999,
AUTHOR = {Lepski, O. V. and Spokoiny, V. G.},
TITLE = {Minimax nonparametric hypothesis testing: the case of an
              inhomogeneous alternative},
JOURNAL = {Bernoulli},
FJOURNAL = {Bernoulli. Official Journal of the Bernoulli Society for
              Mathematical Statistics and Probability},
VOLUME = {5},
YEAR = {1999},
NUMBER = {2},
PAGES = {333--358}
}

@article {li1989,
AUTHOR = {Li, K.-C.},
TITLE = {Honest confidence regions for nonparametric regression},
JOURNAL = {Ann. Statist.},
FJOURNAL = {The Annals of Statistics},
VOLUME = {17},
YEAR = {1989},
NUMBER = {3},
PAGES = {1001--1008}
}
@article{chernozhukov2015valid,
  title={Valid post-selection and post-regularization inference: An elementary, general approach},
  author={Chernozhukov, Victor and Hansen, Christian and Spindler, Martin},
  year={2015},
  publisher={Annual Reviews}
}
@article{belloni2013program,
  title={Program Evaluation and Causal Inference with High-Dimensional Data},
  author={Belloni, Alexandre and Chernozhukov, Victor and Fern{\'a}ndez-Val, Ivan and Hansen, Chris},
  journal={arXiv preprint arXiv:1311.2645},
  year={2013}
}
@article{arias2011global,
  title={Global testing under sparse alternatives: ANOVA, multiple comparisons and the higher criticism},
  author={Arias-Castro, Ery and Cand{\`e}s, Emmanuel J and Plan, Yaniv},
  journal={The Annals of Statistics},
  pages={2533--2556},
  year={2011},
  publisher={JSTOR}
}
@article{laurent2000adaptive,
  title={Adaptive estimation of a quadratic functional by model selection},
  author={Laurent, B and Massart, P},
  journal={The Annals of Statistics},
  volume={28},
  number={5},
  pages={1302--1338},
  year={2000},
  publisher={Institute of Mathematical Statistics}
}

@article{collier2015minimax,
  title={Minimax estimation of linear and quadratic functionals on sparsity classes},
  author={Collier, Olivier and Comminges, La{\"e}titia and Tsybakov, Alexandre B},
  journal={The Annals of Statistics},
  volume={To appear},
  year={2015}
}

@article{guo2018confidence,
  title={Confidence intervals for causal effects with invalid instruments by using two-stage hard thresholding with voting},
  author={Guo, Zijian and Kang, Hyunseung and Tony Cai, T and Small, Dylan S},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={80},
  number={4},
  pages={793--815},
  year={2018},
  publisher={Wiley Online Library}
}

@article{guo2018testing,
  title={Testing endogeneity with high dimensional covariates},
  author={Guo, Zijian and Kang, Hyunseung and Cai, T Tony and Small, Dylan S},
  journal={Journal of Econometrics},
  volume={207},
  number={1},
  pages={175--187},
  year={2018},
  publisher={Elsevier}
}
@article{cai2006optimal,
  title={Optimal adaptive estimation of a quadratic functional},
  author={Cai, T Tony and Low, Mark G},
  journal={The Annals of Statistics},
  volume={34},
  number={5},
  pages={2298--2325},
  year={2006},
  publisher={Institute of Mathematical Statistics}
}
@article{efromovich1996optimal,
  title={On optimal adaptive estimation of a quadratic functional},
  author={Efromovich, Sam and Low, Mark},
  journal={The Annals of Statistics},
  volume={24},
  number={3},
  pages={1106--1125},
  year={1996},
  publisher={Institute of Mathematical Statistics}
}

@article{cai2005nonquadratic,
  title={Nonquadratic estimators of a quadratic functional},
  author={Cai, T Tony and Low, Mark G},
  journal={The Annals of Statistics},
  volume={33},
  number={6},
  pages={2930--2956},
  year={2005},
  publisher={Citeseer}
}
@article{donoho1990minimax,
  title={Minimax quadratic estimation of a quadratic functional},
  author={Donoho, David L and Nussbaum, Michael},
  journal={Journal of Complexity},
  volume={6},
  number={3},
  pages={290--323},
  year={1990},
  publisher={Elsevier}
}
@article{Yang10,
author={Yang, Jian and Benyamin, Beben and McEvoy, Brian P and Gordon, Scott and Henders, Anjali K and Nyholt, Dale R and Madden, Pamela A and Heath, Andrew C and Martin, Nicholas G and Montgomery, Grant W},
title={Common SNPs explain a large proportion of the heritability for human height},
journal={Nature Genetics},
year={2010},
volume={42},
pages={565--569}
}
@article{cai2012direct,
  title={A direct estimation approach to sparse linear discriminant analysis},
  author={Cai, Tony and Liu, Weidong},
  journal={Journal of the American Statistical Association},
  year={2012},
  publisher={Taylor \& Francis}
}
@article{guo2016optimal,
  title={Optimal estimation of co-heritability in high-dimensional linear models},
  author={Guo, Zijian and Wang, Wanjie and Cai, T Tony and Li, Hongzhe},
  journal={arXiv preprint arXiv:1605.07244},
  year={2016}
}
@article{meinshausen2015group,
  title={Group bound: confidence intervals for groups of variables in sparse high dimensional regression without assumptions on the design},
  author={Meinshausen, Nicolai},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={77},
  number={5},
  pages={923--945},
  year={2015},
  publisher={Wiley Online Library}
}
@article{ingster2010detection,
  title={Detection boundary in sparse regression},
  author={Ingster, Yuri I and Tsybakov, Alexandre B and Verzelen, Nicolas},
  journal={Electronic Journal of Statistics},
  volume={4},
  pages={1476--1526},
  year={2010},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{arias2011global,
  title={Global testing under sparse alternatives: ANOVA, multiple comparisons and the higher criticism},
  author={Arias-Castro, Ery and Cand{\`e}s, Emmanuel J and Plan, Yaniv},
  journal={The Annals of Statistics},
  pages={2533--2556},
  year={2011},
  publisher={JSTOR}
}
@article{antoniadis2001regularization,
  title={Regularization of wavelet approximations},
  author={Antoniadis, Anestis and Fan, Jianqing},
  journal={Journal of the American Statistical Association},
  volume={96},
  number={455},
  pages={939--967},
  year={2001},
  publisher={Taylor \& Francis}
}
@misc{owen2012quasi,
  title={Quasi-regression for heritability},
  author={Owen, A},
  year={2012},
  publisher={March}
}
@article{verzelen2016adaptive,
  title={Adaptive estimation of High-Dimensional Signal-to-Noise Ratios},
  author={Verzelen, Nicolas and Gassiat, Elisabeth},
  journal={arXiv preprint arXiv:1602.08006},
  year={2016}
}
@article{bulik2015atlas,
  title={An atlas of genetic correlations across human diseases and traits},
  author={Bulik-Sullivan, Brendan and Finucane, Hilary K and Anttila, Verneri and Gusev, Alexander and Day, Felix R and Loh, Po-Ru and Duncan, Laramie and Perry, John RB and Patterson, Nick and Robinson, Elise B and others},
  journal={Nature genetics},
  volume={47},
  number={11},
  pages={1236--1241},
  year={2015},
  publisher={Nature Research}
}
@article{dicker2014variance,
  title={Variance estimation in high-dimensional linear models},
  author={Dicker, Lee H},
  journal={Biometrika},
  volume={101},
  number={2},
  pages={269--284},
  year={2014},
  publisher={Biometrika Trust}
}
@article{donoho2011noise,
  title={The noise-sensitivity phase transition in compressed sensing},
  author={Donoho, David L and Maleki, Arian and Montanari, Andrea},
  journal={Information Theory, IEEE Transactions on},
  volume={57},
  number={10},
  pages={6920--6941},
  year={2011},
  publisher={IEEE}
}

@article{cai2009data,
  title={A data-driven block thresholding approach to wavelet estimation},
  author={Cai, T. Tony and Zhou, Harrison H},
  journal={The Annals of Statistics},
  volume={37},
  pages={569--595},
  year={2009}}

@article{yi2013sure,
  title={{SURE}-tuned tapering estimation of large covariance matrices},
  author={Yi, Feng and Zou, Hui},
  journal={Computational Statistics \& Data Analysis},
  volume={58},
  pages={339--351},
  year={2013},
  publisher={Elsevier}
}

@article{li1985stein,
  title={From Stein's unbiased risk estimates to the method of generalized cross validation},
  author={Li, Ker-Chau},
  journal={The Annals of Statistics},
  pages={1352--1377},
  year={1985},
  publisher={JSTOR}
}
@article{thrampoulidis2015asymptotically,
  title={Asymptotically Exact Error Analysis for the Generalized $ \ell_2^2$-LASSO},
  author={Thrampoulidis, Christos and Panahi, Ashkan and Hassibi, Babak},
  journal={arXiv preprint arXiv:1502.06287},
  year={2015}
}
@article{bayati2012lasso,
  title={The LASSO risk for Gaussian matrices},
  author={Bayati, Mohsen and Montanari, Andrea},
  journal={Information Theory, IEEE Transactions on},
  volume={58},
  number={4},
  pages={1997--2017},
  year={2012},
  publisher={IEEE}
}
@article{stein1981estimation,
  title={Estimation of the mean of a multivariate normal distribution},
  author={Stein, Charles M},
  journal={The annals of Statistics},
  pages={1135--1151},
  year={1981},
  publisher={JSTOR}
}
@article{donoho1995adapting,
  title={Adapting to unknown smoothness via wavelet shrinkage},
  author={Donoho, David L and Johnstone, Iain M},
  journal={Journal of the american statistical association},
  volume={90},
  number={432},
  pages={1200--1224},
  year={1995},
  publisher={Taylor \& Francis Group}
}
@article{janson2015eigenprism,
  title={EigenPrism: Inference for High-Dimensional Signal-to-Noise Ratios},
  author={Janson, Lucas and Barber, Rina Foygel and Cand{\`e}s, Emmanuel},
  journal={arXiv preprint arXiv:1505.02097},
  year={2015}
}
@article{wainwright2009sharp,
  title={Sharp thresholds for high-dimensional and noisy sparsity recovery using-constrained quadratic programming (Lasso)},
  author={Wainwright, Martin J},
  journal={Information Theory, IEEE Transactions on},
  volume={55},
  number={5},
  pages={2183--2202},
  year={2009},
  publisher={IEEE}
}
@article{raskutti2011minimax,
  title={Minimax rates of estimation for high-dimensional linear regression over-balls},
  author={Raskutti, Garvesh and Wainwright, Martin J and Yu, Bin},
  journal={Information Theory, IEEE Transactions on},
  volume={57},
  number={10},
  pages={6976--6994},
  year={2011},
  publisher={IEEE}
}
@article{chernozhukov2015post,
  title={Post-selection and post-regularization inference in linear models with many controls and instruments},
  author={Chernozhukov, Victor and Hansen, Christian and Spindler, Martin},
  year={2015},
  publisher={MIT Department of Economics Working Paper}
}
@article{blumensath2009iterative,
  title={Iterative hard thresholding for compressed sensing},
  author={Blumensath, Thomas and Davies, Mike E},
  journal={Applied and Computational Harmonic Analysis},
  volume={27},
  number={3},
  pages={265--274},
  year={2009},
  publisher={Elsevier}
}
@article{belloni2012sparse,
  title={Sparse models and methods for optimal instruments with an application to eminent domain},
  author={Belloni, Alexandre and Chen, Daniel and Chernozhukov, Victor and Hansen, Christian},
  journal={Econometrica},
  volume={80},
  number={6},
  pages={2369--2429},
  year={2012},
  publisher={Wiley Online Library}
}
@article{gautier2011high,
  title={High-dimensional instrumental variables regression and confidence sets},
  author={Gautier, Eric and Tsybakov, Alexandre},
  journal={arXiv preprint arXiv:1105.2454v4},
  year={2014}
}
@article{cai2017confidence,
  title={Confidence intervals for high-dimensional linear regression: Minimax rates and adaptivity},
  author={Cai, T Tony and Guo, Zijian},
  journal={The Annals of Statistics},
  volume={45},
  number={2},
  pages={615--646},
  year={2017},
  publisher={Institute of Mathematical Statistics}
}
@article{cai2017supplement,
  title={Supplement to ``Confidence Intervals for High-Dimensional Linear Regression: Minimax Rates and Adaptivity''},
  author={Cai, T Tony and Guo, Zijian},
  journal={The Annals of Statistics},
  year={2017},
}
@article{nickl2013confidence,
  title={Confidence sets in sparse regression},
  author={Nickl, Richard and van de Geer, Sara},
  journal={Annals of Statistics},
  volume={41},
  number={6},
  pages={2852--2876},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@article{cai2018accuracy,
  title={Accuracy assessment for high-dimensional linear regression},
  author={Cai, T Tony and Guo, Zijian},
  journal={Annals of Statistics},
  volume={46},
  number={4},
  pages={1807--1836},
  year={2018},
  publisher={Institute of Mathematical Statistics}
}
@article{cai2016asupplement,
  title={Supplement to ``Accuracy Assessment for High-dimensional Linear Regression"},
  author={Cai, T Tony and Guo, Zijian},
 journal={Annals of Statistics},
  year={to appear},
}


@book{durrett2010probability,
  title={Probability: theory and examples},
  author={Durrett, Rick},
  year={2010},
  publisher={Cambridge university press}
}
@article{zhou2009restricted,
  title={Restricted eigenvalue conditions on subgaussian random matrices},
  author={Zhou, Shuheng},
  journal={arXiv preprint arXiv:0912.4045},
  year={2009}
}
@article{raskutti2010restricted,
  title={Restricted eigenvalue properties for correlated Gaussian designs},
  author={Raskutti, Garvesh and Wainwright, Martin J and Yu, Bin},
  journal={The Journal of Machine Learning Research},
  volume={11},
  pages={2241--2259},
  year={2010},
  publisher={JMLR. org}
}
@article{cai2004adaptation,
  title={An adaptation theory for nonparametric confidence intervals},
  author={Cai, T Tony and Low, Mark G},
  journal={The Annals of statistics},
  volume={32},
  number={5},
  pages={1805--1840},
  year={2005},
  publisher={Institute of Mathematical Statistics}
}
@article{cai2004minimax,
  title={Minimax estimation of linear functionals over nonconvex parameter spaces},
  author={Cai, T Tony and Low, Mark G},
  journal={The Annals of statistics},
  volume={32},
  number={2},
  pages={552--576},
  year={2004},
  publisher={Institute of Mathematical Statistics}
}

@article{belloni2011square,
  title={Square-root lasso: pivotal recovery of sparse signals via conic programming},
  author={Belloni, Alexandre and Chernozhukov, Victor and Wang, Lie},
  journal={Biometrika},
  volume={98},
  number={4},
  pages={791--806},
  year={2011},
  publisher={Biometrika Trust}
}

@article{bickel2009simultaneous,
  title={Simultaneous analysis of Lasso and Dantzig selector},
  author={Bickel, Peter J and Ritov, Ya'acov and Tsybakov, Alexandre B},
  journal={The Annals of Statistics},
  volume={37},
  number={4},
  pages={1705--1732},
  year={2009},
  publisher={JSTOR}
}
@article{ye2010rate,
  title={Rate Minimaxity of the Lasso and Dantzig Selector for the lq Loss in lr Balls},
  author={Ye, Fei and Zhang, Cun-Hui},
  journal={The Journal of Machine Learning Research},
  volume={11},
  pages={3519--3540},
  year={2010},
  publisher={JMLR. org}
}
@article{zhang2014confidence,
  title={Confidence intervals for low dimensional parameters in high dimensional linear models},
  author={Zhang, Cun-Hui and Zhang, Stephanie S},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={76},
  number={1},
  pages={217--242},
  year={2014},
  publisher={Wiley Online Library}
}
@article{van2014asymptotically,
  title={On asymptotically optimal confidence regions and tests for high-dimensional models},
  author={van de Geer, Sara and B{\"u}hlmann, Peter and Ritov, Yaacov and Dezeure, Ruben},
  journal={The Annals of Statistics},
  volume={42},
  number={3},
  pages={1166--1202},
  year={2014},
  publisher={Institute of Mathematical Statistics}
}
@article{javanmard2014confidence,
  title={Confidence intervals and hypothesis testing for high-dimensional regression},
  author={Javanmard, Adel and Montanari, Andrea},
  journal={The Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={2869--2909},
  year={2014},
  publisher={JMLR. org}
}
@article{javanmard2013hypothesis,
  title={Hypothesis testing in high-dimensional regression under the gaussian random design model: Asymptotic theory},
  author={Javanmard, Adel and Montanari, Alessandro},
  journal={Information Theory, IEEE Transactions on},
  volume={60},
  number={10},
  pages={6522--6554},
  year={2014},
  publisher={IEEE}
}
@article{cai2012optimal,
  title={Optimal rates of convergence for sparse covariance matrix estimation},
  author={Cai, T Tony and Zhou, Harrison H },
  journal={The Annals of Statistics},
  volume={40},
  number={5},
  pages={2389--2420},
  year={2012},
  publisher={Institute of Mathematical Statistics}
}


@article{ren2015asymptotic,
  title={Asymptotic normality and optimalities in estimation of large Gaussian graphical models},
  author={Ren, Zhao and Sun, Tingni and Zhang, Cun-Hui and Zhou, Harrison H},
  journal={The Annals of Statistics},
  volume={43},
  number={3},
  pages={991--1026},
  year={2015},
  publisher={Institute of Mathematical Statistics}
}

@article{verzelen2012minimax,
  title={Minimax risks for sparse regressions: Ultra-high dimensional phenomenons},
  author={Verzelen, Nicolas},
  journal={Electronic Journal of Statistics},
  volume={6},
  pages={38--90},
  year={2012},
  publisher={Institute of Mathematical Statistics}
}

@article{cai2011constrained,
  title={A constrained
  $\ell_1$ minimization approach to sparse precision matrix estimation},
  author={Cai, T Tony and Liu, Weidong and Luo, Xi},
  journal={Journal of the American Statistical Association},
  volume={106},
  number={494},
  pages={594--607},
  year={2011},
  publisher={Taylor \& Francis}
}
@article{golub1996matrix,
  title={Matrix computations. 1996},
  author={Golub, Gene H and Van Loan, Charles F},
  journal={Johns Hopkins University, Press, Baltimore, MD, USA},
  pages={374--426},
  year={1996}
}

@article{tibshirani1996regression,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society. Series B (Methodological)},
  volume={58},
  number={1},
  pages={267--288},
  year={1996},
  publisher={JSTOR}
}
@article{candes2007dantzig,
  title={The Dantzig selector: statistical estimation when p is much larger than n},
  author={Cand{\`e}s, Emmanuel and Tao, Terence},
  journal={The Annals of Statistics},
  volume={35},
  number={6},
  pages={2313--2351},
  year={2007},
  publisher={JSTOR}
}
@article{sun2012scaled,
  title={Scaled sparse linear regression},
  author={Sun, Tingni and Zhang, Cun-Hui},
  journal={Biometrika},
  volume={101},
  number={2},
  pages={269--284},
  year={2012},
  publisher={Biometrika Trust}
}
@article{chandrasekaran2012convex,
  title={The convex geometry of linear inverse problems},
  author={Chandrasekaran, Venkat and Recht, Benjamin and Parrilo, Pablo A and Willsky, Alan S},
  journal={Foundations of Computational mathematics},
  volume={12},
  number={6},
  pages={805--849},
  year={2012},
  publisher={Springer}
}
@article{liu2013gaussian,
  title={Gaussian graphical model estimation with false discovery rate control},
  author={Liu, Weidong},
  journal={The Annals of Statistics},
  volume={41},
  number={6},
  pages={2948--2978},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@article{liuhypothesis,
  title={Hypothesis Testing for High-dimensional Regression Models},
  author={Liu, Weidong and Luo, Shan}
}
@article{nickl2013confidence,
  title={Confidence sets in sparse regression},
  author={Nickl, Richard and van de Geer, Sara},
  journal={The Annals of Statistics},
  volume={41},
  number={6},
  pages={2852--2876},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@article{batir2008inequalities,
  title={Inequalities for the gamma function},
  author={Batir, Necdet},
  journal={Archiv der Mathematik},
  volume={91},
  number={6},
  pages={554--563},
  year={2008},
  publisher={Springer}
}
@book{boucheron2013concentration,
  title={Concentration inequalities: A nonasymptotic theory of independence},
  author={Boucheron, St{\'e}phane and Lugosi, G{\'a}bor and Massart, Pascal},
  year={2013},
  publisher={OUP Oxford}
}
@incollection{vershynin2010introduction,
  author      = {Vershynin, Roman},
  title       = {Introduction to the non-asymptotic analysis of random matrices},
  editor      = {Yonina Eldar and Gitta Kutyniok},
  booktitle   = {Compressed Sensing: Theory and Applications},
  publisher   = {Cambridge University Press},
  pages={210--268},
  year        = {2012}
}
@book{buhlmann2011statistics,
  title={Statistics for high-dimensional data: methods, theory and applications},
  author={B{\"u}hlmann, Peter and Van De Geer, Sara},
  year={2011},
  publisher={Springer Science \& Business Media}
}
@article{ning2017general,
  title={A general theory of hypothesis tests and confidence regions for sparse high dimensional models},
  author={Ning, Yang and Liu, Han},
  journal={The Annals of Statistics},
  volume={45},
  number={1},
  pages={158--195},
  year={2017},
  publisher={Institute of Mathematical Statistics}
}
@article{neykov2015unified,
  title={A Unified Theory of Confidence Regions and Testing for High Dimensional Estimating Equations},
  author={Neykov, Matey and Ning, Yang and Liu, Jun S and Liu, Han},
  journal={arXiv preprint arXiv:1510.08986},
  year={2015}
}
@article{zhu2017projection,
  title={A projection pursuit framework for testing general high-dimensional hypothesis},
  author={Zhu, Yinchu and Bradic, Jelena},
  journal={arXiv preprint arXiv:1705.01024},
  year={2017}
}
@article{javanmard2017flexible,
  title={A Flexible Framework for Hypothesis Testing in High-dimensions},
  author={Javanmard, Adel and Lee, Jason D},
  journal={arXiv preprint arXiv:1704.07971},
  year={2017}
}
